Restricting Control Flow During Speculative Execution with Venkman

Side-channel attacks such as Spectre that utilize speculative execution to steal application secrets pose a significant threat to modern computing systems. While program transformations can mitigate some Spectre attacks, more advanced attacks can divert control flow speculatively to bypass these protective instructions, rendering existing defenses useless. In this paper, we present Venkman: a system that employs program transformation to completely thwart Spectre attacks that poison entries in the Branch Target Buffer (BTB) and the Return Stack Buffer (RSB). Venkman transforms code so that all valid targets of a control-flow transfer have an identical alignment in the virtual address space; it further transforms all branches to ensure that all entries added to the BTB and RSB are properly aligned. By transforming all code this way, Venkman ensures that, in any program wanting Spectre defenses, all control-flow transfers, including speculative ones, do not skip over protective instructions Venkman adds to the code segment to mitigate Spectre attacks. Unlike existing defenses, Venkman does not reduce sharing of the BTB and RSB and does not flush these structures, allowing safe sharing and reuse among programs while maintaining strong protection against Spectre attacks. We built a prototype of Venkman on an IBM POWER8 machine. Our evaluation on the SPEC benchmarks and selected applications shows that Venkman increases execution time to 3.47$\times$ on average and increases code size to 1.94$\times$ on average when it is used to ensure that fences are executed to mitigate Spectre attacks. Our evaluation also shows that Spectre-resistant Software Fault Isolation (SFI) built using Venkman incurs a geometric mean of 2.42$\times$ space overhead and 1.68$\times$ performance overhead.

==> future.tex <==
%%=============================================================================
\section{Future Work}
\label{section:future}
%%=============================================================================

Several directions exist for future work.  First, we will
improve {\System}'s precision.  {\System} currently ensures that
speculative execution adheres to a very conservative
control flow graph.  More sophisticated code placement strategies might allow
{\System} to restrict speculative calls to a set of specific
call targets or returns to a specific set of call sites.
Second, we will investigate whether transformations like
super-block construction~\cite{AllenKennedy}
and
if-conversion~\cite{AllenKennedy}
can reduce the number of fences that {\System} inserts by
creating more straight-line code.
Finally, we will port {\System} to x86 and ARM.

%Second, we will explore hardware acceleration for {\System}.
%Adding a constant bit-mask operand to
%branches may reduce {\System}'s code size overheads.
%Going further, if software can communicate to hardware which branches
%can target which code locations, the processor could ensure that such
%restrictions are observed when performing branch target prediction.
%This would allow safe BTB and RSB sharing but alleviate the need to created
%aligned basic blocks.


==> tables/clamav-baseline.tex <==
\begin{table}[tb]
\centering
\caption{ClamAV Baseline Execution Time}
\label{table:clamav-baseline}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|r|r||r|r|}
\hline
  {\bf File Size (KB)} & {\bf Time (ms)} & {\bf File Size (KB)} & {\bf Time (ms)} \\
\hline
  1 & 73.3
  &
  1,024 & 145.7
  \\
\hline
  2 & 73.5
  &
  2,048 & 219.5
  \\
\hline
  4 & 74.2
  &
  4,096 & 147.2
  \\
\hline
  8 & 73.8
  &
  8,192 & 655.1
  \\
\hline
  16 & 74.5
  &
  16,384 & 552.1
  \\
\hline
  32 & 74.4
  &
  32,768 & 1031.3
  \\
\hline
  64 & 75.2
  &
  65,536 & 1987.7
  \\
\hline
  128 & 76.1
  &
  131,072 & 3898.1
  \\
\hline
  256 & 78.0
  &
  262,144 & 7720.2
  \\
\hline
  512 & 83.0
  &
  524,288 & 9351.1
  \\
\hline
\end{tabular}
}
\end{table}


==> tables/gnupg-encrypt-baseline.tex <==
\begin{table}[tb]
\centering
\caption{GnuPG Encryption Baseline Execution Time}
\label{table:gnupg-encrypt-baseline}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|r|r||r|r|}
\hline
  {\bf File Size (KB)} & {\bf Time (ms)} & {\bf File Size (KB)} & {\bf Time (ms)} \\
\hline
  1 & 8.2
  &
  256 & 49.8
  \\
\hline
  2 & 8.3
  &
  512 & 91.7
  \\
\hline
  4 & 8.6
  &
  1,024 & 176.2
  \\
\hline
  8 & 8.9
  &
  2,048 & 345.8
  \\
\hline
  16 & 9.9
  &
  4,096 & 684.8
  \\
\hline
  32 & 12.0
  &
  8,192 & 1363.1
  \\
\hline
  64 & 17.2
  &
  16,384 & 2722.2
  \\
\hline
  128 & 27.9
  &
  32,768 & 5433.1
  \\
\hline
\end{tabular}
}
\end{table}

